Consistent Identity Association for Open-Vocabulary Counting in Videos

Open-vocabulary video object counting asks how many distinct instances of a text-specified category appear across a video. Recent approaches combine promptable detection with tracking and count the resulting identities in the video. However, occlusions, re-entry, and fragmented trajectories can cause trackers to issue new identities to objects already counted. To address this issue, we present Consistent Identity Association (CIA), a lightweight association module that decouples identity counting from tracker outputs. Whenever the underlying tracker issues new identities, CIA jointly determines whether the corresponding detections represent new objects, returning instances, or duplicates of active tracks. This consistent identity assignment reduces repeated counting. We also introduce the Video Counting Benchmark (VCB), comprising 951 videos and 1,639 queries, with instance identities for evaluating whether objects are counted once. We instantiate CIA with a frozen SAM 3 tracker and evaluate it on VCB and VideoCount. On BURST-Count, Dance-Count and GMOT-Count, CIA reduces count MAE by 60%, 63% and 13% relative to CountVid, and by 3%, 68% and 19% relative to SAM3Count, respectively. Code is available at https://github.com/Joan947/CIA.

==> sec/7_llm_statement.tex <==
\section*{LLM Usage Statement}

Across all the sections, we used two AI tools. \emph{Claude} (Anthropic), a large language model, helped us plan the paper's structure and draft it, which the authors then revised. \emph{Grammarly} (its AI writing assistance) was used to correct grammar. The authors take full responsibility for all content.

